A comparison of online search engine autocompletion in Google and Baidu

Warning: This paper contains content that may be offensive or upsetting. Online search engine auto-completions make it faster for users to search and access information. However, they also have the potential to reinforce and promote stereotypes and negative opinions about a variety of social groups. We study the characteristics of search auto-completions in two different linguistic and cultural contexts: Baidu and Google. We find differences between the two search engines in the way they suppress or modify original queries, and we highlight a concerning presence of negative suggestions across all social groups. Our study highlights the need for more refined, culturally sensitive moderation strategies in current language technologies.

==> backup.tex <==
% chinese language for OpenAI

In our study, we analyzed the common social groups featured in autocomplete suggestions on Baidu and Google, with the numerical distribution of these groups in each category presented in Table \ref{tab:comparison_baidu_google}. Additionally, Figure \ref{fig:top10_common_groups} details the inconsistencies observed in the top 10 responses from each search engine.





\begin{table}[h]
\centering
\begin{tabular}{lrr}
\hline
\textbf{Category} & \textbf{Baidu } & \textbf{Google} \\ \hline

Age               & 56                    & 11                     \\
Gender            & 169                   & 106                    \\
Lifestyle         & 8                     & 39                     \\
Nationalities     & 124                   & 89                     \\
Peoples           & 50                    & 9                      \\
Political         & 15                    & 6                      \\
Religion          & 15                    & 1                      \\
\hline
\end{tabular}
\caption{Baidu vs. Google: A Comparative Overview of Common Group Counts}

\label{tab:comparison_baidu_google}
\end{table}


Then, we will move to an analysis of the negative analysis of the auto-completion part of Baidu and Google. 

Our study was concentrated on two key sentiment metrics: \textit{Completion Sentiment} and \textit{Full Suggestion Sentiment} See detailed in Figure \ref{fig:combined_sentiment_full_suggestion}.

\begin{itemize}
    \item \textbf{Completion Sentiment Analysis:} This analysis highlighted notable differences in the negative review distribution between Baidu and Google. Specifically, the 'Peoples' and 'Political' categories showed a higher proportion of negative reviews in one engine over the other. This discrepancy suggests a variation in user perception and presentation of these categories in search suggestions.

    \item \textbf{Full Suggestion Sentiment Analysis:} Trends observed here were akin to those in the Completion Sentiment. The disparities in negative review ratios were more evident, hinting that the entirety of suggestions might significantly affect user sentiment. Categories like 'Nationalities' and 'Lifestyle' exhibited marked differences in negative sentiment distribution, implying distinct representation biases in each search engine.
\end{itemize}



\begin{figure}[htbp]
    \centering
    % Adjust the widths to fit within half an A4 page
    %\includegraphics[width=0.45\textwidth]{Sentiment.png}
    % Space between the two images
    \vspace{10pt}  
    %\includegraphics[width=0.45\textwidth]{full_suggestion.png}
    \caption{Top: Negative Review Proportions in Baidu vs. Google Based on Completion Sentiments. Bottom: Negative Review Proportions in Baidu vs. Google Based on Full Suggestion}
    \label{fig:combined_sentiment_full_suggestion}
\end{figure}

\subsubsection{Fisher's Exact Test Results}
The Fisher's Exact Test provided statistical backing to our sentiment analysis. See Table \ref{tab:fishers_test}:
\begin{itemize}
    \item \textbf{Full Suggestion Test Results:} Significant variances were observed in categories like 'Nationalities' (Odds Ratio: 3.0819, P-value: 0.00014) and 'Peoples' (Odds Ratio: 7.4375, P-value: 0.0213), indicating a statistically notable difference in representation in search suggestions of Baidu and Google.

    \item \textbf{Completion Test Results:} The Completion analysis also showed significant findings, particularly in the 'Nationalities' category, which had an Odds Ratio of 2.3386 and a P-value of 0.0056, underscoring the difference in the portrayal of nationalities in search completions.
\end{itemize}

\begin{table}[H]
\centering
\small % Smaller font size for the table
\setlength{\tabcolsep}{2pt} % Further reduce the space between columns
% Full Suggestion Table
\begin{minipage}[t]{0.4\linewidth} % Reduced width
\centering
\begin{tabular}{>{\raggedright\arraybackslash}p{2.1cm} >{\raggedright\arraybackslash}p{1cm} >{\centering\arraybackslash}p{1.1cm}}
\multicolumn{3}{c}{\textbf{Part I: Full Suggestion}} \\
\hline
\textbf{Category} & \textbf{Odds Ratio} & \textbf{P-value} \\ 
\hline
Gender            & 0.9418              & 0.8884           \\
Nationalities     & 3.0819              & 0.00014          \\
Religion          & inf                 & 0.1875           \\
Age               & 2.9841              & 0.2036           \\
Peoples           & 7.4375              & 0.0213           \\
Lifestyle         & 1.4286              & 0.7155           \\
Political         & 4.0000              & 0.2906           \\
\hline
\end{tabular}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.4\linewidth} % Reduced width
\centering
\begin{tabular}{|>{\centering\arraybackslash}p{1.1cm} >{\centering\arraybackslash}p{1.1cm}}
\multicolumn{2}{c}{\textbf{Part II: Completion}} \\
\hline
\textbf{Odds Ratio} & \textbf{P-value} \\ 
\hline
1.0057              & 1.0000           \\
2.3386              & 0.0056           \\
inf                 & 1.0000           \\
2.7564              & 0.1494           \\
inf                 & 0.0008           \\
0.5700              & 0.7008           \\
1.3750              & 1.0000           \\
\hline
\end{tabular}
\end{minipage}
\captionof{table}{Fisher's Exact Test Results (Full Suggestion and Completion)}
\label{tab:fishers_test}
\end{table}



Our analysis indicates that despite Google's robust moderation policies, high negative sentiment ratios persist in categories like 'Gender', suggesting these measures may not be uniformly effective across all content types. Similarly, Baidu, shaped by different regulatory and cultural frameworks, shows significant negative sentiment in the same categories, despite having less comprehensive moderation policies than Google. 

\begin{figure*}[htbp]
    \centering
    % %\includegraphics[width=0.8\textwidth]{whole_groups_distribution.png}
    \caption{Comparative Sentiment Distribution Across Social Groups in Baidu and Google}
    \label{fig:sentiment_distribution}
\end{figure*}

Our sentiment analysis across various social groups in Baidu and Google is detailed in Figure \ref{fig:sentiment_distribution}. Despite Google's stricter moderation policies, both search engines display considerable negative sentiment in categories like 'Age' and 'Gender'. This pattern suggests that the current moderation strategies may not sufficiently counteract negative biases or stereotypes. While Baidu and Google implement moderation policies, their effectiveness in addressing negative sentiment within social groups seems to differ notably.


\section{Limitations}
Our research has certain limitations. Firstly, we adapted social groups from a U.S.-centric study, which may not fully represent global perspectives. Secondly, search engine auto-completions are subject to change over time and vary according to each search engine's policies. Thirdly, our use of a single template for collecting search engine auto-completions limits the scope of stereotypes we could capture for each category.

Despite these limitations, we believe our research is significant. To our knowledge, this is the first study to investigate stereotypes moderation policies cross different serach engines about Chinese people and compare them across English and Chinese languages in , as well as between the U.S. and mainland China. 

\section{Conclusion}

This study provides a critical insight into the moderation strategies of autocomplete suggestions in two major search engines, Baidu and Google, highlighting the significant influence of cultural, linguistic, and regulatory contexts. 

Our findings indicate the persistence of negative stereotypes, especially in categories like 'Gender' and 'Age',despite the efforts of both search engines to moderate content, This suggests that current moderation practices may not be sufficiently countering negative biases. 

% chinese language for OpenAI
